Towards Practical Privacy-Preserving Solution for Outsourced Neural Network Inference

When neural network model and data are outsourced to cloud server for inference, it is desired to preserve the confidentiality of model and data as the involved parties (i.e., cloud server, model providing client and data providing client) may not trust mutually. Solutions were proposed based on multi-party computation, trusted execution environment (TEE) and leveled or fully homomorphic encryption (LHE/FHE), but their limitations hamper practical application. We propose a new framework based on synergistic integration of LHE and TEE, which enables collaboration among mutually-untrusted three parties, while minimizing the involvement of (relatively) resource-constrained TEE and allowing the full utilization of the untrusted but more resource-rich part of server. We also propose a generic and efficient LHE-based inference scheme as an important performance-determining component of the framework. We implemented/evaluated the proposed system on a moderate platform and show that, our proposed scheme is more applicable/scalable to various settings, and has better performance, compared to the state-of-the-art LHE-based solutions.

==> backprop.tex <==

\section{Backward Propagation}

% When summing up, 
% one vector is divided into two and then rotate 

For each layer $l$,
let $\nabla\tilde{C}^{(l)}_i$ for $i\in\{0,\cdots,\iota_l-1\}$
denote the $i$-th ciphertext for the gradient of input, and
$\nabla\tilde{C}^{(l+1)}_i$ for $i\in\{0,\cdots,o_l-1\}$
denote the $i$-th ciphertext for the gradient of output.


\subsection{Final Layer}



\subsection{Backward Propagation: Fully-connected Layer $l$}

The design of backward propagation is mainly driven by the following goals:
\begin{itemize}
    \item 
    The workload at the TEE is minimized even at the cost of (reasonably) increasing the cost at the untrusted server. 
    \item 
    The workload at the untrusted server should be lowered and paralleled as much as possible.   
\end{itemize}
%
Here, we also consider two types of fully-connected layers the same as the above. 
However, in contrary to the forward propagation, 
we describe these types based on how many sets of outputs are encoded per ciphertext.

\subsubsection{Type I: Single Set of Outputs per Ciphertext}

This type corresponds to Type I presented in Section~\ref{sec:forward-full-1}.

\paragraph{Backward Propagation}

The backward propagation algorithm is formally presented in
Algorithm~\ref{alg:bwd-full-layer-I}.

\begin{algorithm}[htb]
\caption{Backward Prop. through Fully-connected Layer $l$ (Type I)}
\label{alg:bwd-full-layer-I}

\begin{algorithmic}[1]
\For{$i\in\{0,\cdots,\iota'_l-1\}$}
    \State $\nabla\tilde{C}^{(l)}_i\leftarrow 0$
    \For{$j\in\{0,\cdots,o_l-1\}$}     
        \State $\nabla\tilde{C}^{(l)}_i = \nabla\tilde{C}^{(l+1)}_{j}\bigodot\tilde{M}^{(l)}_{j,i}$
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}



\paragraph{Weight Update}

Weight updating goes through the following steps:
\begin{itemize}
    \item 
    Step 1 - The gradient for each $\tilde{M}^{(l)}_{i,j}$, 
    denoted as $\nabla\tilde{M}^{(l)}_{i,j}$, is computed as $\nabla\tilde{C}^{(l+1)}_i\bigodot\tilde{C}^{(l)}_j$.
    \item 
    Step 2 - For each $\nabla\tilde{M}^{(l)}_{i,j}$, 
    where $i\in\{0,\cdots,o_l-1\}$ and $j\in\{0,\cdots,\iota'_l-1\}$,
    the elements of each n-element set is added up to the element of index $i\cdot\iota'_l+j$;
    then it is multiplied with the vector that encodes $0$'s and $1$'s where
    1 only appears at each position $p$ such that $p~\mod~n~=~i\cdot\iota'_l+j$. 
    \item 
    Step 3 - The ciphertexts resulted from the above step are split into $n$-element groups.
    \item 
    Step 4 - The ciphertexts in the same group are added up (merged such that non-zero elements are only added with zeros).
    \item 
    Step 5 - The ciphertexts resulted from the above step are decrypted by the TEE and then re-encrypted.
    \item 
    Step 6 - Each of the ciphertexts resulted from the above are split into $n$ ciphertexts (reverse of Step 4). 
    \item 
    Step 7 - For each of the ciphertexts resulted from the above,
    the non-zero element at each $n$-element set is populated (duplicated) to all the positions of the set.
    \item 
    Step 8 - Each of the ciphertexts from the above step is added to the current weight ciphertext, respectively,
    to obtain the updated weight ciphertexts. 
\end{itemize}
Note that, the TEE is involved only in step 5. 



\subsubsection{Type II: Multiple Set of Outputs per Ciphertext}

\paragraph{Backward Propagation}
Algorithm~\ref{alg:bwd-full-layer-II} formally presents the algorithm for computing the gradients of input
from the gradients of output through backward propagation at layer $l$.

\begin{algorithm}[htb]
\caption{Backward Prop. through Fully-connected Layer $l$ (Type II)}
\label{alg:bwd-full-layer-II}
\begin{algorithmic}[1]
\For{$i\in\{0,\cdots,\iota_l-1\}$}
    \State $\nabla\tilde{C}^{(l)}_i\leftarrow 0$ 
    \For{$j\in\{0,\cdots,\lceil\frac{o_l\cdot n}{s}\rceil-1\}$}     
        \State $\nabla\tilde{C}^{(l)}_i += \nabla\tilde{C}^{(l+1)}_j\bigodot\tilde{M}^{(l)}_{j,i}$
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


\paragraph{Weight Update}
(similar to the Type I) 




\subsection{Background Propagation: Pooling Layer $l$}



\subsection{Background Propagation: Convolutional Layer $l$}


\paragraph{Backward Propagation}
The backward propagation algorithm is formally presented in Algorithm~\ref{alg:bwd-conv-layer}.

\begin{algorithm}[htb]
\caption{Backward Prop. through Convolutional Layer $l$}
\label{alg:bwd-conv-layer}

\begin{algorithmic}[1]

\For{$i\in\{0,\cdots,\alpha-1\}$} \Comment{each channel $i$}
    \For{$j\in\{0,\cdots,\iota_l\}$} \Comment{each input matrix $j$}
        % \For{$k\in\{0,\cdots,f_l-1\}$} \Comment{each filter matrix $k$}
        \For{$u\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$}
            \For{$v\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$} 
                \For{$x\in\{0,\cdots,\gamma_l-1\}$}
                    \For{$y\in\{0,\cdots,\gamma_l-1\}$}
                        \State $u'\leftarrow u\cdot\delta_l)$
                        \State $v'\leftarrow v\cdot\delta_l$
                        \State $\nabla\tilde{C}^{(l,j)}_{i,u+x,v+y} \leftarrow 0$
                        \For{$k\in\{0,\cdots,f_l-1\}$} \Comment{each filter matrix $k$}
                            \State $\nabla\tilde{C}^{(l,j)}_{i,u+x,v+y} += \nabla\tilde{C}^{(l+1,j\cdot f_l+k)}_{i,u',v'}\bigodot\hat{F}^{(l,k)}_{i,x,y}$
                        \EndFor
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
\EndFor

\end{algorithmic}
\end{algorithm}

\paragraph{Weight Update}
Weight updating goes through the following steps:
\begin{itemize}
    \item 
    Algorithm~\ref{alg:weight-gradient-conv-layer} is applied to compute the weight gradients.
    \item 
    For the set of $\nabla\tilde{F}^{(l,k)}_{i,x,y}$ where $k\in\{0,\cdots,f_l-1\}$, 
    channel $i\in\{0,\cdots,\alpha-1\}$,
    and $x,y\in\{0,\cdots,\gamma_l-1\}$, 
    the afore-described weight update procedure is applied to 
    update the filters with the minimal facilitation from the TEE. 
\end{itemize}

\begin{algorithm}[htb]
\caption{Computing Weight Gradients for Convolutional Layer $l$}
\label{alg:weight-gradient-conv-layer}

\begin{algorithmic}[1]

\For{$i\in\{0,\cdots,\alpha-1\}$} \Comment{each channel $i$}
    \For{$j\in\{0,\cdots,\iota_l\}$} \Comment{each input matrix $j$}
        \For{$k\in\{0,\cdots,f_l-1\}$} \Comment{each filter matrix $k$}
            \For{$x\in\{0,\cdots,\gamma_l-1\}$}
                \For{$y\in\{0,\cdots,\gamma_l-1\}$}
                    \State $\nabla\tilde{F}^{(l,k)}_{i,x,y}\leftarrow 0$
                    \For{$u\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$}
                        \For{$v\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$}
                        \State $u'\leftarrow u\cdot\delta_l$
                        \State $v'\leftarrow v\cdot\delta_l$
                        \State $\nabla\tilde{F}^{(l,k)}_{i,x,y} += \nabla\tilde{C}^{(l+1,j\cdot f_l+k)}_{i,u,v}\bigodot\tilde{C}^{(l,j)}_{i,u'+x,v'+y}$
                        \EndFor
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
\EndFor

\end{algorithmic}
\end{algorithm}










==> integrity.tex <==
\section{Scheme for Testing Computation Integrity}
\label{sec:integrity}


